Light WIMPs and MeV Gamma-ray Detection with COSI

Light weakly interacting massive particles (WIMPs), whose masses are in the sub-GeV scale, have been attracting more attention due to the negative results searching for traditional WIMPs. The light WIMPs are expected to produce gamma rays from annihilation in the MeV energy region. Advancements in technology have opened up possibilities to precisely detect MeV gamma rays, leading to the upcoming space-based mission of the Compton Spectrometer and Imager (COSI). We comprehensively and quantitatively study the phenomenology of light WIMPs to determine if the COSI observations will probe their viable model parameter regions. We first construct models to describe light WIMPs based on the minimality and renormalizability of quantum field theory. Next, we impose various constraints on the models obtained from cosmological observations (CMB, BBN) and dark matter searches (accelerator, underground, astrophysical experiments, etc.). Finally, we identify viable parameter regions in each model and discuss whether or not COSI will be sensitive to the parameter regions. We find that a velocity-dependent annihilation cross-section is predicted in some regions, enabling COSI to detect the dark matter signal while avoiding severe constraints from cosmological observations.

==> Tmp/Accerelator.tex <==
%While the parameter region where the mediator particle decays into the visible (invisible) final states with a branching ratio greater than 99\% is depicted as blue points, the intermediate region where the mediator particle decays both visibly and invisibly with substantial branching ratios is expressed as red points indicating the utilization of a less reliable method.


==> Tmp/CoreCusp.tex <==
%As seen in Fig.\,\ref{fig: core-cusp}, the self-interacting cross-section should be enhanced at $v \sim 10^{-3}$ to solve the core-cusp problem. In s-channel resonant models with invisible decay modes, $v_R$ is constrained to be larger than $\sim 10^{-2.5},$ and we numerically checked that these parameters cannot address the core-cusp problem through DM collisions alone.

%Lastly, we consider the small-scale crisis. Though the self-interacting cross-section should be enhanced at $v \sim 10^{-3}$ to solve the core-cusp problem, in s-channel resonant models with visible decay modes, $\sqrt{\delta}$ is constrained to be larger than $\sim 10^{-2}$. We numerically checked that these parameters cannot address the core-cusp problem through DM collisions alone.

==> Tmp/Lyalpha.tex <==
\subsubsection{Limit on the WIMP from the Lyman-\texorpdfstring{$\alpha$}{TEXT} observation}
\label{subsubsec: Lyman}

As seen in the left panel of Fig.\,\ref{fig: BBN-photo}, when the WIMP mass is smaller than $\sim 2$\,MeV, the BBN observation does not constrain the annihilation cross-section even if the cross-section is boosted by the $s$-channel resonance of the mediator particle. On the other hand, the observation of the Lyman-$\alpha$ forest constrains the cross-section even in such a case. Residual neutral hydrogen atoms in the intergalactic medium produce a series of absorption lines in the spectrum of a background source (e.g., a quasar) through the scattering in the $n = 1 \to 2$ Lyman-$\alpha$ transition, known as the `Lyman-$\alpha$ forest.' Since the distribution of the neutral hydrogen atoms in the universe is attributed to that of the light WIMP, the observation of the Lyman-$\alpha$ forest can be used to constrain the light WIMP scenarios as follows: When the WIMP remains in kinetic equilibrium with photons until the late universe, the power spectrum is suppressed at the small scale due to the dark Silk damping. According to numerical simulations\,\cite{Vogelsberger:2015gpr}, the power spectrum was found to have the cutoff at the scale of
\begin{equation}
    M_{\rm cut} \simeq
    5 \cdot 10^{10} \left( \frac{T_{\rm kd}}{100\,{\rm eV}} \right)^{-3}
    h^{-1} M_\odot,
\end{equation}
where $T_{\rm kd}$ is the kinetic decoupling temperature and $M_\odot$ is the mass of the sun. On the other hand, the SDSS-III BOSS collaboration recently measured the power spectra of quasars that are distributed at the redshift of 2--5 and found the cutoff satisfy $M_{\rm cut}/M_\odot \lesssim 10^{10}$\,\cite{Chabanier:2018rga, Bringmann:2016ilk}. This result, therefore, indicates that the temperature should satisfy $T_{\rm kd} \gtrsim 200$\,eV\,\cite{Bringmann:2016ilk}.

In the light WIMP scenarios discussed in this article, the WIMP mainly interacts with electrons and positrons via the mediator particle, so it kinematically decouples from the cosmic plasma when the electron density in the universe is suppressed enough, i.e., when the temperature of the universe is much higher than 200\,eV. So, the constraint from observing the Lyman-$\alpha$ forest is safely satisfied. The exception is the case that the WIMP annihilates through the $s$-channel resonance of the mediator particle, i.e., {\bf SS-R}, {\bf FS-R}, {\bf SV-R}, {\bf FV-R}, {\bf SV(B)-R}, and {\bf FV(B)-R} scenarios. In these scenarios, when the difference between the mass of the mediator particle and twice the WIMP mass is small enough, the annihilation cross-section is larger as the temperature of the WIMP is smaller, even in the late universe. This means the WIMP with a lower momentum has a larger annihilation cross-section. So, after the freeze-out, WIMPs with lower momenta keep annihilating more efficiently than those with higher momenta, making the WIMP temperature effectively larger, hence the cutoff scale $M_{\rm cut}$ larger than those in the non-resonant scenarios\,\cite{Binder:2017rgn}. When the WIMP is heavier than $\sim 2$\,MeV in the resonance scenarios, thanks to the BBN constraint discussed in section\,\ref{subsubsec: BBN on annihiation}, the annihilation cross-section is already suppressed when the temperature of the universe is $T_\gamma \sim 200$\,eV, so the Lyman-$\alpha$ constraint is safely satisfied. On the other hand, the WIMP mass can be smaller than $\sim 2$\,MeV in the {\bf SV-R} and {\bf FV-R} scenarios, and the annihilation cross-section may not be suppressed even at the temperature $T_\gamma \sim 200$\,eV.

So, we impose the Lyman\,$\alpha$ constraint on the {\bf SV-R} and {\bf FV-R} scenarios as follows: The WIMP annihilation cross-section averaged by the WIMP velocity distribution function already starts decreasing when the temperature of the universe is 200\,eV. It seems a cursory constraint compared to the others discussed in this section. However, parameter regions limited by this constraint are more severely constrained by indirect dark matter detection, even if we include various associated uncertainties. So, we impose the Lyman\,$\alpha$ constraint and discard such parameter regions in advance to make our analysis less time-consuming.

%We also impose an additional constraint on the SV-R and FV-R scenarios, which is from the Lyman-$\alpha$ observation; it is imposed for the convenience of making numerical analysis less time-consuming, for it is always weaker than that of the indirect dark matter detection, as stated in section\,\ref{subsubsec: Lyman}.

%Furthermore, regarding the constraint from the SN neutrino observation, we do not impose it in our analysis but deal with a referential one, as mentioned in section\,\ref{subsubsec: other constraints}.
